SkeletonNet: A Topology-Preserving Solution for Learning Mesh Reconstruction of Object Surfaces from RGB Images

This paper focuses on the challenging task of learning 3D object surface reconstructions from RGB images. Existingmethods achieve varying degrees of success by using different surface representations. However, they all have their own drawbacks,and cannot properly reconstruct the surface shapes of complex topologies, arguably due to a lack of constraints on the topologicalstructures in their learning frameworks. To this end, we propose to learn and use the topology-preserved, skeletal shape representationto assist the downstream task of object surface reconstruction from RGB images. Technically, we propose the novelSkeletonNetdesign that learns a volumetric representation of a skeleton via a bridged learning of a skeletal point set, where we use paralleldecoders each responsible for the learning of points on 1D skeletal curves and 2D skeletal sheets, as well as an efficient module ofglobally guided subvolume synthesis for a refined, high-resolution skeletal volume; we present a differentiablePoint2Voxellayer tomake SkeletonNet end-to-end and trainable. With the learned skeletal volumes, we propose two models, the Skeleton-Based GraphConvolutional Neural Network (SkeGCNN) and the Skeleton-Regularized Deep Implicit Surface Network (SkeDISN), which respectivelybuild upon and improve over the existing frameworks of explicit mesh deformation and implicit field learning for the downstream surfacereconstruction task. We conduct thorough experiments that verify the efficacy of our proposed SkeletonNet. SkeGCNN and SkeDISNoutperform existing methods as well, and they have their own merits when measured by different metrics. Additional results ingeneralized task settings further demonstrate the usefulness of our proposed methods. We have made both our implementation codeand the ShapeNet-Skeleton dataset publicly available at ble at https://github.com/tangjiapeng/SkeletonNet.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> method_figures/related_old.tex <==
\section{Related Works}

In this section, we review existing methods of deep learning surface reconstruction from RGB images. We focus on the mesh representation of object surface, while other representations, e.g., point set or volume, are briefly discussed as well. We organize the review into two lines of methods that either explicitly learn deformation of mesh vertices, or learn an implicit surface representation from which the surface mesh can be extracted. We finally discuss existing research where the interior shape representation of skeleton is used for various downstream tasks.

\subsection{Implicit Surface Generator}
\noindent \textbf{\emph{Learning Voxels}} 
    Voxels, extended from pixels, are usually used in the form of binary values or signed distances to represent a 3D shape. Because of its regularity, most of existing deepnets-based shape analysis ~\cite{wu20153d, brock2016generative} or shape generation ~\cite{choy20163d, girdhar2016learning, wu2016learning, kar2017learning} methods adopt it as the primary representation. For example, the work of ~\cite{choy20163d} combines 3D convolutions and long short-term memory (LSTM) units to achieve volumetric grid reconstruction from single-view or multi-view RGB images. A 3D auto-encoder is trained in ~\cite{girdhar2016learning}, whose decoder part is used to build the mapping from a 2D image to a 3D occupancy grid. Wu et al. ~\cite{wu2016learning} adopts the generative adversarial networks \cite{goodfellow2014generative}, frequently used in image translation tasks, to contribute a better volume-based shape reconstruction. These methods tend to predict a low-resolution volumetric grid due to the high computational cost of 3D convolution operators. Based on the observation that only a small portion of regions around the boundary surface contain the shape information, the octree representation has been employed in recent shape analysis works ~\cite{riegler2017octnet, wang2017cnn, wang2018adaptive} for efficient computation. Although these methods enable generating high-resolution volumes, the complicated data structure of the octree makes the training very hard. The outputs thus usually contain artifacts. 
   % {\color{blue}
   % In terms of shape generation, Tatarchenko at al. ~\cite{tatarchenko2017octree} designs an Octree Generating Networks (OGN) to simultaneously estimate the octree structure and its contents. Only octants around boundary regions are further processed by up-convolution operations to improve the accuracy of reconstructed regions in those octants, which can achieve  high resolution reconstructions with less requirements of time and memory. Hierarchical Surface Prediction (HSP) ~\cite{hane2017hierarchical} follows the similar idea to exploit the sparsity of 3D surface through octree structure. The octree decoder implemented in OGN is explored in breadth-first manner, but that HSP explore the implementation in depth-first manner. In our work, we aim to generate the surface mesh of the object instead of its solid volume. As its efficiency and topology-insensitivity, we also leverage volume-based generator to convert the inferred skeletal point cloud to a solid volume, effectively bridging the gap between the skeletal points and the surface mesh. 
   % }
   \newline

\noindent \textbf{\emph{Learning Implicit Functions}}
A shape can also be represented using a continuous implicit function which usually has two ways of discretization: an in-out field or a signed distance field (SDF). With this representation, a clean surface mesh can be easily extracted using the method of marching cube \cite{lorensen1987marching}. According to the principle that multi-layer feed-forward networks can approximate arbitrary functions in theory  \cite{hornik1989multilayer}, a lot of recent works attempt to utilize the multi-layer perceptrons(MLPs) to approximate the desired implicit function. The works of \cite{chen2019learning, mescheder2019occupancy, michalkiewicz2019deep, saito2019pifu} choose to learn the in-out field where the 3D surface is considered to be a continuous decision boundary of the inside or outside classification. The methods of \cite{park2019deepsdf, xu2019disn} strive to SDF prediction, so they can not only decide whether points are inside or outside but also how far they are from the target surface. Concretely, these approaches firstly extract latent shape embedding from the input image, and then employ MLPs-based decoders to predict the functional values for the given 3D points. Owning to the continuity of implicit representation, their reconstructions are often smooth and can ideally achieve infinite resolution. The usage of local features from the input image in DISN \cite{xu2019disn} can further effectively help the recovery of fine-grained details. {\color{red} BSP-Net \cite{chen2020bsp} can directly infer polygon mesh without applying marching cubes although it also learns an implicit field. It interpretes the network parameters to define the hyper-planes, and then reconstructs a shape by combining them. Similarly, based on the knowledge that a ReLU based MLP partitions its input space into a number of linear regions, Lei. et al \cite{lei2020analytic} proposes an analytic marching algorithm to identify zero-level surface parallelly. }  However, it is still challenge for them to reconstruct shapes with complex topologies. This is because they don't incorporate explicit structure inference in their learning process.  


In this work, we firstly propose a deep learning-based method that explicitly learns the skeleton from the input image. Taking the produced skeletal information as a guidance, a novel strategy is also invented to predict more accurate implicit field. \newline

    %{\color{blue} 
    %An implicit surface representation such as signed distance field(SDF) and in-out field is defined by a continuous function over 3D space. Then a surface mesh can be extracted from a desired iso-surface of the implicit field by applying the marching cubes algorithm \cite{lorensen1987marching}. 
    %The works of \cite{chen2019learning, mescheder2019occupancy, michalkiewicz2019deep, saito2019pifu} choose to learn the in-out field where 3D surface is considered to be a continuous decision boundary for inside or outside classification. The methods of \cite{park2019deepsdf, xu2019disn} strive to SDF prediction, so they can not only decide whether points are inside or outside but also how far they are from the target surface.  
    
    
    %Concretely, they firstly extract latent shape embedding from the input image, and then employ MLPs-based decoders to predict the functional values for the given 3D points.  Compared with octree-based generators \cite{tatarchenko2017octree, riegler2017octnetfusion, hane2017hierarchical, wang2018adaptive}, they bypass the complex implementations and avoid the issues of large memory requirement and long training time. %although they need to spend more time on infernce. 
    
    % In order to overcome this limitation, we extract multi-scale skeleton-aware features from produced skeleton to provide structure guidance. The contained structure information in skeletons can compensate the shape properties understood directly from the input image, and promote topology preservation to improve the accuracy of the predicted implicit field.
    %}
    

\subsection{Explicit Surface Generator}
\noindent \textbf{\emph{Learning Points}}
Point cloud, sampled from the objects' surfaces and formed by a set of points, is one of the most popular representations of 3D shapes. As a pioneer work, Fan et al. ~\cite{fan2017point} proposes to directly learn a deep regression model for generating coordinates of points from single-view images. Chamfer distance (CD) or Earth Mover's distance (EMD) is involved for building the training loss. To improve the plausibility of the generated point clouds, point-based discriminators are utilized by Jiang et al. \cite{jiang2018gal} and Achlioptas et al. \cite{achlioptas2018learning}. There also exists some approaches ~\cite{tatarchenko2016multi, arsalan2017synthesizing, lin2018learning} that take multi-view depth maps as the output representation, where image-based generative models can be used for depth maps synthesis. A point cloud can be obtained by a direct fusion from the depth images. Although the generated point cloud can capture the rough shape, it is usually noisy, making extracting a clean surface from it extremely challenging. As one of the core components in the proposed method, we also need to regress the skeletal points from an image. The difficulties of existing point-based generators are alleviated in the following ways: 1) Due to the compactness of the skeleton, regressing skeletal points is easier than regressing the points over the surface. 2) Based on the observation that a skeleton is usually consisting of curve-like and surface-like points, a novel parallel network design is developed to respectively generating the two kinds of points. 3) The inferred skeletal points are only an intermediate output, which will further be refined and used to provided guidance for final surface generation.\newline
   
   % {\color{blue}  
   % Wang et al. utilizes EdgeConv \cite{wang2019dynamic} to exploit neighborhood information across points so that they can alleviate local minima. 
   % A similar coarse-to-fine framework is employed in \cite{pan2018residual}.
   % Chen et. al \cite{chen2020deep} proposes a graph-filtering module to refine the coarse results attained from the deformation of a uniform 2D lattice by the folding module \cite{yang2018foldingnet}.
   %  Multi-view depth maps are used as the output representation in ~\cite{tatarchenko2016multi, arsalan2017synthesizing, lin2018learning}, which are generated using image generative models and then fused to a dense point cloud. Based on geometry image representation, a kind of spherical parametrization of 3D surfaces, the work of ~\cite{sinha2017surfnet} also turns the 3D shape reconstruction problem into a image generation task.  Nevertheless, due to the nature of regressing large scale points, the predicted points are still of low accuracy and large noise, which causes the difficulty of acquiring manifold mesh via post-processing steps. In our method, we employ point cloud fitting techniques to generate skeleton point cloud firstly, due to the ease of capturing correct topologies. The usage of parametric line and square elements eases the approximating of the diverse local structures.} 
    
\noindent \textbf{\emph{Learning Meshes}}
Mesh, as the most natural discretization of a manifold surface, has been widely used in many graphics applications. Due to its irregular structure, conventional CNN is difficult to be directly applied for mesh generation. To alleviate this challenge, ~\cite{kato2018neural, wang2018pixel2mesh} take an initial sphere or ellipsoid as template and attempt to learn the vertex deformations to approximate the target surfaces with maintaining the face connectivity relationships. Limited by the spherical topology, they cannot deal with those models with non-zero genus. Although \cite{jack2018learning, wang20193dn} enlarge the search range of template into a set of reference models, their reconstructions are still not topology-free. Several recent methods are thus proposed to tackle this challenge. For example, Atlasnet ~\cite{groueix2018atlasnet} learns to use a set of square lattices to fit the target surface. Although this method is not topology-restricted, it tends to cause non-closed meshes with severe self-intersections. Pan et al. \cite{pan2019deep} presents TM-Net which dynamically updates the mesh connectivity when deforming the template sphere. The topology modification is achieved by a face removal mechanism where triangles whose estimated errors are larger than a predefined threshold are pruned. This is further improved by Nie et al. \cite{nie2020total3dunderstanding} with a novel adaptive thresholding strategy. However, these two approaches are still hard to deal with shapes with complex topologies, especially those with thin structures (like the chair in Fig. \ref{fig:show_alg}).       

In this work, we aim to not only output a clean closed mesh but also capture the correct topology. By involving a procedure of skeleton learning, we propose a method for explicitly mesh generation. Due to the decoupling of structure inference and geometric details, the proposed approach shows significantly better capability of handling complex shapes than existing methods. 
    
    
   % {\color{blue}  To handle the topology sensitive reconstruction, TMNet \cite{pan2019deep} dynamically updates the connectivity relationships when deforming the template sphere. The topology modification is achieved by the face removal mechanism where triangles whose estimated errors are larger than a predefined threshold will be pruned. Although Nie et al. \cite{nie2020total3dunderstanding} improve the robustness through edge removal, it is still highly likely to remove triangles mistakenly. As a consequence, the occurrences of wrong removal can destroy topology and surface geometry because it is nontrivial to determine an appropriate threshold to adapt a wide range of object models.  Moreover, it is still difficult to handle the recovery of these models with many loops and holes like the chair in Fig. \ref{fig:show_alg}.}

\subsection{Skeleton as an Interior Shape Representation}

    % \subsection{Structure Inference}
    % Another research topic related to our work is learning to infer structure of objects. All existing works in this field utilize primitives or parts to represent the structures. As a pioneer work, the method of ~\cite{Tulsiani_2017_CVPR} proposes an approach to learn an assembling of cuboid primitives to fit the input shape, in an unsupervised learning fashion. Concurrently, a recurrent neural network is exploited by Zou et al. ~\cite{Zou_2017_ICCV} to sequentially predict the primitives from a single depth map. By representing the man-made shapes with hierarchical organization of semantic parts, the method presented in ~\cite{li_sig17} can generate both the part shapes and their relationships which forms the output shapes of the objects. The same decoder can also be adopted for structure generation from single images, as implemented in ~\cite{niu2018im2struct}. The binary-tree based recursive decoder is further extended to N-ary case in the work of StructureNet \cite{mo2019structurenet}. Most recently, a seq2seq network \cite{wu2019pq} is also utilized for sequentially predicting the parts. Although these approaches have witnessed the possibility to infer part/primitive-based structures using deep learning techniques, they are still challenge to handle complex shapes. Another drawback of them is the requirement of a large-scale human-annotated dataset. 
    
    % Different from them, in this work, we use meso-skeleton to represent the shape structure which is more general and much easier to obtain from the models. 
    The medial axis transform (MAT) \cite{blum1967transformation} is a intrinsic shape representation including the medial axis together with the associated radius function of the maximally inscribed spheres, which can be used to reconstruct the original shape. A lot of methods \cite{attali1996modeling, chazal2005lambda, miklos2010discrete} are designed to compute or approximate the MAT for downstream applications, like shape recognition, modeling and editing. For example, Q-MAT \cite{li2015q}  and Q-MAT+ \cite{pan2019q} acquire geometrically accurate, structurally simple, and compact MAT meshes, which can employed as supervision to constraint the MAT learning from point clouds \cite{yang2020p2mat}. Concurrently, MAT-Net \cite{hu2019mat} uses their computed MAT to perform 3D object classification.
    Skeletal shape representation \cite{au2008skeleton, cao2010point, bucksch2010skeltre}, as  a compact point cloud, is a kind of medial axis transformation. Curve skeleton extraction techniques play important roles in the context of surface reconstruction \cite{sharf2007fly, tagliasacchi2009curve, huang2013l1}. In order to be adaptive with different topologies (2D sheets & 1D curves), the work of \cite{tagliasacchi2012mean} aim to compute meso-skeletons from surface point clouds, which combine medial sheets and curve skeletons. After the construction of meso-skeleton, Wu. et al \cite{wu2015deep} exploits its contained context to complete missing regions on surfaces. Most recently, P2PNet \cite{yin2018p2p} introduces a bi-directional point displacement network to learn geometric transformations between meso-skeletons and surfaces.
     
    In our work, we use meso-skeleton to explicitly represent the shape topology. To the best of knowledge, we are the first one to explore skeleton inference from RGB images. To do this, we firstly extract meso-skeletons for ShapeNet dataset \cite{chang2015shapenet} based on the method of \cite{wu2015deep}. The recovered skeleton can provide structure guidance for further learning of surface mesh generation.

==> tables/emd.tex <==
% \setlength{\tabcolsep}{4pt}
\begin{table*}[t]
 \renewcommand\arraystretch{1.2}
 \begin{center}
    \begin{tabular}{*{13}{c}}
       \toprule
       \multirow{2}*{Category} & \multicolumn{6}{c}{Implicit}   & \multicolumn{6}{c}{Explicit} \\
       \cmidrule(lr){2-7} \cmidrule(lr){8-13}
       & R2N2 & OGN &  IMNet & OccNet  & DISN & Ours & PSG & N3MR & P2M  & AtlasNet &TMNet & Ours\\
       \midrule
       \midrule
       plane   & 8.255  & 9.039 & 12.081 & \textbf{8.050} & 11.010 & 10.843
               & 10.841  & 8.909  &9.339 & 7.225  & 5.948 & \textbf{5.081} \\
       
       bench   & 7.667  & 8.883  &  8.443  & \textbf{5.840} & 8.306 & 8.267
               & 11.457  & 13.756 &7.812 & 9.436 & 6.163 & \textbf{5.675} \\
               
       cabinet & 7.980 & 8.404  &  8.525  & \textbf{6.671} & 8.185 & 8.486
               & 15.264 & 20.742  &7.172 & 8.016  & \textbf{6.589} & 8.339
               \\
               
       car  & 9.381 & 6.060  & 11.249   &\textbf{5.883} & 11.235  & 11.268
            & 11.679 & 12.994  &8.379  & 7.015  & 6.200  & \textbf{6.170}
            \\
            
       chair & 8.472 & 9.066 &  8.767 &  \textbf{6.571} & 8.328  & 8.196
             & 12.877 & 13.371 &  8.352  & 7.965  & 6.738 & \textbf{6.368}
             \\
             
       monitor & 6.425 & 7.102 &  9.592  & \textbf{5.876} & 8.801 & 8.905
               & 13.456 & 15.978  &7.694  & 7.852 & 6.468 & \textbf{6.179}
               \\
               
       lamp & 11.697 & 11.383 & 13.275  & 11.908 & 11.983 & \textbf{11.646}   
               & 19.573 & 16.331  &11.054 & 10.341 & 10.958 & \textbf{8.568}
               \\
               
       speaker   & 8.453 & 9.148 &  9.279 & \textbf{7.672} & 8.403 & 8.305
               & 17.696 & 18.832 &  9.778  & 8.808 & \textbf{7.371} & 8.083
               \\
               
       firearm & 6.577 & \textbf{6.052} &  8.653 & 6.891 & 7.057 & 7.047
               &12.984 & 13.794  &6.062  & 7.047 & 6.135 & \textbf{4.499}
               \\
               
       couch   &7.078 & 7.987 &  7.635  & \textbf{5.486} & 6.684  & 6.707
               & 12.956 & 16.688 & 7.368  & 8.427  & \textbf{5.765} & 6.401
               \\
       table   &8.164 & 9.316 &   11.350  & \textbf{6.836} & 10.263 & 10.176
               & 13.220 & 15.55  &  9.662 & 9.529 & \textbf{7.540} & 7.645
               \\
       
       cellphone  &6.245 & 4.941 & 5.163  & \textbf{3.976} & 4.936 & 5.034
               & 13.555 & 21.557  & 4.506 & 7.415  & \textbf{3.887} & 4.913
               \\
               
       watercraft &6.6833 &8.098 & 10.245  & \textbf{7.743}  & 9.523 & 9.414
               & 12.333 &13.135  & 8.315  & 7.086 & 7.114 & \textbf{6.195}
               \\
       \midrule
       mean    & 8.017  & 8.114 &  9.558 & \textbf{6.877}  & 8.859  & 8.792 
               & 13.684  &15.511 & 8.115  & 8.166 & 6.683 & \textbf{6.470}\\
       \bottomrule
      \end{tabular}
      \caption{Quantitative comparisons (Earth mover's distance($\times 100$)) of our method against state-of-the-arts. The lower is better. }
    \label{Tab:emd}
 \end{center}
\end{table*}
%\setlength{\tabcolsep}{1.4pt}
